Vulnerable GPU Memory Management: Towards Recovering Raw Data from GPU

In this paper, we present that security threats coming with existing GPU memory management strategy are overlooked, which opens a back door for adversaries to freely break the memory isolation: they enable adversaries without any privilege in a computer to recover the raw memory data left by previous processes directly. More importantly, such attacks can work on not only normal multi-user operating systems, but also cloud computing platforms. To demonstrate the seriousness of such attacks, we recovered original data directly from GPU memory residues left by exited commodity applications, including Google Chrome, Adobe Reader, GIMP, Matlab. The results show that, because of the vulnerable memory management strategy, commodity applications in our experiments are all affected.

==> defense.tex <==
\section{Discussion}
\label{defense}
\vspace{2pt}\noindent{\bf GPU memory compression.} Various GPU memory compression methods have been designed in recent years to reduce the size of color data in memory and use the limited memory bandwidth more efficiently. Although the data in physical memory space is compressed and the similarity between image rows and columns are reduced, it does not affect our attack result. In fact, the compression is guaranteed to be transparent to the upper-layer applications. So, no matter how pixels are compressed in the physical memory, our application is able to read the decompressed version of images.

%In this section, the paper proposes 2 potential countermeasures that mitigate the danger brought by video memory leakage. The first strategy doesn't touch the GPGPU framework while the later one requires manufacture to do a little modification to their frameworks. Before we start to discuss the countermeasures, some observations are stated. Firstly, users cannot afford the price of zeroing all the video memory automatically by GPU. Secondly, developers are too lazy to zero out sensitive memory by themselves.

%The first observation, accepted by predecessors \cite{leakageweb,di2013cuda,LeeKKK14}, make manufacture impossible to deploy a zeroing mechanism similar to what used in main memory, because bandwidth has been one of the bottle neck in today's GPU architecture while zeroing video memory before allocation makes the precious bandwidth even more tight. Similarly, zeroing all the memory by developers are neither preferred because of the performance derogation.

%The later observation is partially because developers have gotten used to free memory directly without consideration to leakage in CPU model. As a result, it is very difficult to guarantee that all application developers can clear all sensitive memory before deletion though big company can use code analysis tools to guarantee so.

%We then propose two potential countermeasures without proof as follow.

\vspace{2pt}\noindent{\bf Limitations.} %Our proposed algorithm performs well during the evaluation test. But, we can not find a strict mathematical proof for it. Besides, the pseudo-periodicity does fail in some specific case, say the pure color images or random images.
We chose four applications of interest for evaluation and demonstrate the efficacy of our attack. We did not evaluate more applications due to the large amount of manual work involved in running victim applications in different settings and examining result. However, we believe our result is sufficient enough to demonstrate the unneglectable security issue underlying GPU memory management framework. The information extraction process is not fully automated yet. So far, we only apply text and face recognition for the images rendered by Chrome. We are investigating more feasible ways for this task. Though our approach is fairly robust if the image is loaded into memory without extra processing by the victim applications, the parallel rendering technique used by applications like Chrome raises the bar for images recovering. It is possible to stitch together the image segments and we are in the process of exploring feasible algorithms, e.g., puzzle-solving algorithm. Yet, the leaked information from the segments is already alarming.
\ignore{
\vspace{2pt}\noindent{\bf Mitigation.} Naturally, one would come up with a mitigation approach that automatically clears the used pages in global and all private memory after the program exits. This solution should mitigate the threats in theory, but is hard to be adopted virtually. The performance degradation comes with this solution is huge, as identified in previous works~\cite{leakageweb,di2013cuda,LeeKKK14}. More specifically, clearing the entire memory would incur two times more overhead during GPU context switching~\cite{LeeKKK14}. As follows, we present two possible solutions which prevent GPU memory leaks without much impact to performance.

\vspace{2pt}\noindent{\bf Manual clearing.}
%Without touching the GPGPU framework and GPU driver, manufacture or 3rd party organization could develop a series of code check tools that list memories not zeroed out before deletion by modifying the existing memory checking tools. To maximally reduce the impact to performance, developers can selectively let memories that they think non-sensitive alone and clear those sensitive only.
%Admittedly, common developers may not check their codes before releasing, which still gives adversary opportunities to steal leakages. However, we argue that users of most popular GPU accelerated application can be protected if only big companies release their applications after carefully checking. Considering the quality of developers in those companies, guaranteeing confidentiality should not be so big a problem. The attacking coverage will be much squashed imaging that popular applications leaks only non-sensitive data.
Since complete and dynamic residue cleaning requires a lot of resources and brings in performance degradation, selectively clearing is a more practical solution.  Given that the GPU structure cannot be completely redesigned in a short time, developers should manually clear the memory before releasing it. To maximally protect performance, they can devote resources to clear those memory regions containing user's sensitive data only. \ignore{The fundamental reason behind the GPU leaks lies in that the developers forget to clear the delete memory after use.} Such request, however, is hard to be fulfilled by every developer, especially when the applications maintained have colossal code base (e.g., Chrome). Similar problem also exists in CPU structure and the issues around memory leaks from CPU have been well studied and many approaches have been proposed. A developer could use static analyzer to pinpoint the location in code where memory is not freed~\cite{Cherem2007, Hastings91purify} or identify the leaks in the runtime through monitoring the stacks or heaps~\cite{Xu2008, Novark2009}. We hope the ideas in those research could be leveraged to build detectors against GPU leaks. \ignore{If considering the issue of performance degradation, the detectors could assign priorities of fixing and let developers decide whether or not to free memory.}

%\vspace{2pt}\noindent{\bf Selective memory clearing.}
%The memory requested by application by default are not cleared automatically nowadays. We recommend that GPU manufactures modify their frameworks to support automatically memory clearing before releasing by default while developers highly demanding on performance can disable the automatical clearing for sensitive memories via API added by manufacture.
%Different from existing mechanism where developers need to pick those sensitive memories out and protect them, this measure by default protects all memories no matter if it is sensitive or not. Naturally, developers will remove protections to those non-sensitive and resource consuming memories for performance optimization.
%This scheme holds some outstanding advantages.
%Firstly, it is highly compatible to the developed projects. Obviously, this protection doesn't affect any correctness of existing projects. So after users updated the driver and frameworks to the latest version, the security concerns can be relieved, and with the application's updating, the performance can go back to normal level.
%Secondly, for developers, it requests only little security knowledge. Developers often have a strong background on performance optimization but not inevitably a strong awareness to protect users' privacy, so, it is relatively an easier work for developers.
%In case the program is not checked, GPU needs to take care of the residues as a last line of defense. Wiping out all private memory and used global memory has performance issue and we recommend memory to be selectively cleared. Regarding managing the memory associated with CPU, garbage collection is broadly embraced by modern programming languages to automatically free unused memory. However, this feature is not presented in GPU computing. In the long run, we advocate that a finer-grained approach needs to be proposed to manage the unused memory of GPU. In defending against the attacks discussed in this paper, there is an alternative way. Our attack exploits the similarity between consecutive rows and columns, which can be intentionally reduced by GPU: GPU can randomly inject noise or sparsely remove certain region of memory to break such correlation. Adding noise has been proved to be an effective way to mitigate side-channel attacks, e.g., against web applications~\cite{Luo2011} and we believe it can be adopted for this problem.

\vspace{2pt}\noindent{\bf Image layout obfuscation.}
%Memory layout randomization is a widely used method to protect users from buffer overflow attacks \cite{Random}. The principle can be borrowed to countermeasure the consequence of GPU memory leakage. memory belonging to a process could be permutated according to a rule while different processes use different rules. In this case, the later processes could get the consecutive pixels only if the previous randomization rule could be acquired. One of the most important assumption of our scheme is that there should be high geographical relatedness between consecutive columns and rows. Without the geographical relatedness resulted from layout randomization, attackers could hardly recover meaningful images. However, this method may increase the accessing delay, because of the newly introduced memory address translation time.
The above solution does not mitigate the problem completely. Even best code analyzer or developer cannot capture every code location processing sensitive data. Alternatively, we suggest obfuscate the image layout in GPU memory. \ignore{Memory layout randomization is a widely used method to protect users from buffer overflow attacks \cite{Random}. The principle can be followed here.} When an application delivers an image to GPU, it could intentionally store the pixels into irregular format instead of a sequential array. The routine of obfuscation can be implemented in the complier or system library managing GPU memory. The key assumption of our scheme is that there should be high geographical correlation between consecutive columns and rows. Apparently, the correlation is interrupted by layout obfuscation. This scheme would introduce some overhead inevitably, but comparing with blindly filling zeros, the overhead should be smaller as only images go through this additional step. The technique may weaken the performance of memory compression, because the obfuscation breaks local redundancy of the image which makes compression ratio worse.

\vspace{2pt}\noindent{\bf Defense for virtual machine.}
To defend attacker from virtualized platform, it is sufficient for the hypervisor to clear the whole GPU memory space every time before the VM start for now. The overhead in this case is negligible, because: 1) memory only needs to be cleaned when VM switching happens. 2) VM switching already takes a lot of time and the extra overhead is thus not prominent. So, we recommend all cloud service providers with GPU support in their infrastructure to clean GPU memory during VM switching.

}

